Generalizing Dataset Distillation via Deep Generative Prior

Dataset Distillation aims to distill an entire dataset's knowledge into a few synthetic images. The idea is to synthesize a small number of synthetic data points that, when given to a learning algorithm as training data, result in a model approximating one trained on the original data. Despite recent progress in the field, existing dataset distillation methods fail to generalize to new architectures and scale to high-resolution datasets. To overcome the above issues, we propose to use the learned prior from pre-trained deep generative models to synthesize the distilled data. To achieve this, we present a new optimization algorithm that distills a large number of images into a few intermediate feature vectors in the generative model's latent space. Our method augments existing techniques, significantly improving cross-architecture generalization in all settings.

==> _macros.tex <==






\newcommand{\nbf}[1]{{\noindent \textbf{#1.}}}

\newcommand{\supp}{supplemental material\xspace}
\ifarxiv \renewcommand{\supp}{appendix\xspace} \fi

\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}

\newcommand{\R}[1]{{%
    \textbf{%
        \ifstrequal{#1}{1}{\textcolor{red}{R#1}}{%
        \ifstrequal{#1}{2}{\textcolor{blue}{R#1}}{%
        \ifstrequal{#1}{3}{\textcolor{magenta}{R#1}}{%
        \ifstrequal{#1}{4}{\textcolor{teal}{R#1}}{%
                           \textcolor{cyan}{R#1}%
        }}}}%
    }%
}}

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{2pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{packed_item}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{2pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}



\usepackage{amsmath,amsfonts,bm,relsize,dsfont}
\usepackage[numbers,sort&compress]{natbib}
\usepackage{anyfontsize}


\algrenewcommand{\algorithmicrequire}{\textbf{Input:}}
\algrenewcommand{\algorithmicensure}{\textbf{Output:}}

\definecolor{MyDarkBlue}{rgb}{0.02,0.02,0.8}
\definecolor{MyDarkGreen}{rgb}{0.02,0.6,0.02}
\definecolor{MyDarkRed}{rgb}{0.8,0.02,0.02}
\definecolor{MyDarkOrange}{rgb}{0.40,0.2,0.02}
\definecolor{MyPurple}{RGB}{111,0,255}
\definecolor{MyRed}{rgb}{1.0,0.0,0.0}
\definecolor{MyGold}{rgb}{0.75,0.6,0.12}
\definecolor{MyDarkgray}{rgb}{0.66, 0.66, 0.66}
\definecolor{MyDarkCyan}{rgb}{0.05, 0.55, 0.45}
\definecolor{MyBlack}{rgb}{0., 0., 0.}
\definecolor{MyMagenta}{rgb}{1., 0., 1.}
\definecolor{BerkeleyYellow}{RGB}{255,204,41}
\definecolor{BerkeleyLightBlue}{RGB}{94,146,221}
\definecolor{BkDarkBlue}{rgb}{.05,.07,.353}

\definecolor{MyDarkGray2}{rgb}{0.6, 0.6, 0.6}
\newcommand{\gray}[1]{\textcolor{MyDarkGray2}{#1}}


\newcommand{\junyanz}[1]{\emph{\textcolor{MyDarkGreen}{JZ: #1}}}
\newcommand{\richard}[1]{\emph{\textcolor{MyDarkOrange}{RZ: #1}}}
\newcommand{\eli}[1]{\emph{\textcolor{MyDarkGreen}{ES: #1}}}
\newcommand{\nupur}[1]{\emph{\textcolor{MyDarkBlue}{NK: #1}}}
\newcommand{\george}[1]{\emph{\textcolor{MyRed}{GC: #1}}}
\newcommand{\VS}[1]{\emph{\textcolor{MyGold}{VS: #1}}}
\newcommand{\added}[1]{\textcolor{MyMagenta}{#1}}
\newcommand{\camready}[1]{#1}

\newcommand{\suppmat}[1]{\textcolor{MyBlack}{#1}}


\newcommand{\red}[1]{\textcolor{MyRed}{#1}}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}

\NewDocumentCommand{\anote}{}{\makebox[0pt][l]{$^*$}}

\def\L{\mathcal{L}} %
\def\v{\mathbf{v}} %
\def\x{\mathbf{x}} %
\def\y{\mathbf{y}} %
\def\z{\mathbf{z}} %

\def\vpos{\bm{v^{+}}} %
\def\vneg{\bm{v^{-}}} %

\def\X{\mathcal{X}} %
\def\Y{\mathcal{Y}} %
\def\Z{\mathcal{Z}} %
\def\data{\mathcal{D}} %
\def\P{\mathbb{P}} %

\def\xhat{{\hat{\x}}}
\def\yhat{{\hat{\y}}}
\def\zhat{{\hat{\z}}}

\def\xtilde{{\tilde{\x}}}
\def\ytilde{{\tilde{\y}}}
\def\ztilde{{\tilde{\z}}}

\def\xbar{{\bar{\x}}}
\def\ybar{{\bar{\y}}}
\def\zbar{{\bar{\z}}}

\def\xstar{{\x^{*}}}
\def\ystar{{\y^{*}}}
\def\zstar{{\z^{*}}}


\def\D{{D_{\phi}}}
\def\G{{G_{\theta}}}
\def\Re{\mathds{R}}
\newcommand{\expect}[1]{\mathbb{E}_{#1}}
\def\NCE{\ell}

\def\dc{\texttt{DC}}
\def\glad{\texttt{GLaD}}
\def\dsa{\texttt{DSA}}
\def\dm{\texttt{DM}}
\def\mtt{\texttt{MTT}}
\def\tesla{\texttt{TESLA}}
\def\pkmn{Pokémon}

\newcommand{\fid}{Fr\'echet Inception Distance\xspace}



\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}


\newcommand{\seg}{\rvs_c}
\newcommand{\repr}{\rvr}
\newcommand{\repru}{\repr_{u, \sP}}
\newcommand{\uprepru}{\repr_{u, \sP}^{\uparrow}}
\newcommand{\f}{f}
\newcommand{\h}{h}



\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}

\newcommand{\reffig}[1]{Figure~\ref{fig:#1}}
\newcommand{\refsec}[1]{Section~\ref{sec:#1}}
\newcommand{\refapp}[1]{Appendix~\ref{sec:#1}}
\newcommand{\reftbl}[1]{Table~\ref{tbl:#1}}
\newcommand{\refalg}[1]{Algorithm~\ref{alg:#1}}
\newcommand{\refline}[1]{Line~\ref{line:#1}}
\newcommand{\shortrefsec}[1]{\S~\ref{sec:#1}}
\renewcommand{\refeq}[1]{Eqn.~\ref{eq:#1}}
\newcommand{\refeqshort}[1]{(\ref{eq:#1})}
\newcommand{\shortrefeq}[1]{\ref{eq:#1}}
\newcommand{\lblfig}[1]{\label{fig:#1}}
\newcommand{\lblsec}[1]{\label{sec:#1}}
\newcommand{\lbleq}[1]{\label{eq:#1}}
\newcommand{\lbltbl}[1]{\label{tbl:#1}}
\newcommand{\lblalg}[1]{\label{alg:#1}}
\newcommand{\lblline}[1]{\label{line:#1}}
\newcommand{\ignorethis}[1]{}
\newcommand{\revision}[1]{\color{black}#1\color{black}}
\newcommand{\myitem}{\vspace{-5pt}\item}
\newcommand{\myparagraph}[1]{\vspace{1pt} \noindent \textbf{#1} \ }
\newcommand{\mysubsection}[1]{\vspace{1mm}\noindent{\bf #1}}


\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}

\newcommand{\image}{{\rvx}}
\newcommand{\latent}{{\rvz}}
\newcommand{\images}{{\mathcal{X}}}
\newcommand{\imagedist}{{p_{\text{data}}(\image)}}
\newcommand{\latentdist}{{p(\latent)}}
\newcommand{\imageD}{{D_X}}
\newcommand{\Fnet}{{F}}
\newcommand{\sketch}{{\rvy}}
\newcommand{\sketches}{{\mathcal{Y}}}
\newcommand{\sketchdist}{{p_{\text{data}}(\sketch)}}
\newcommand{\sketchD}{{D_Y}}
\newcommand{\modelold}{{G(\rvz; \theta)}}
\newcommand{\modelnew}{{G(\rvz; \theta')}}
\newcommand{\losssketch}{{\mathcal{L}_{\text{sketch}}}}
\newcommand{\lossimage}{{\mathcal{L}_{\text{image}}}}
\newcommand{\lossweight}{{\mathcal{L}_{\text{weight}}}}

\newcommand{\method}{{GAN Sketching}}

\newcommand{\pdata}{{D}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\Ls}{\mathcal{L}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak




\newcommand{\xpar}[1]{\noindent\textbf{#1}\ \ }
\newcommand{\vpar}[1]{\vspace{3mm}\noindent\textbf{#1}\ \ }

\newcommand{\shapenet}{ShapeNet\xspace}
\newcommand{\pascal}{PASCAL 3D+\xspace}

\newcommand{\degree}{\ensuremath{^\circ}\xspace}
\newcommand{\ignore}[1]{}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\fcseven}{$\mbox{fc}_7$}

\renewcommand*{\thefootnote}{\arabic{footnote}}


\def\naive{na\"{\i}ve\xspace}
\def\Naive{Na\"{\i}ve\xspace}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{e.g\onedot,\xspace} 
\def\Eg{E.g\onedot,}
\def\ie{i.e\onedot,\xspace} 
\def\Ie{\emph{I.e}\onedot,}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother



\newcommand*{\img}[1]{%
    \raisebox{-.25\baselineskip}{%
        \includegraphics[
        height=\baselineskip,
        width=\baselineskip,
        keepaspectratio,
        ]{#1}%
    }%
}

\fboxsep=0mm%
\fboxrule=2pt%
\newcommand*{\myoverpic}[2]{
  \begin{overpic}[width=.18\linewidth]{#1}
     \put(60,63){\fbox{\includegraphics[width=.06\linewidth]{#2}}}  
  \end{overpic}
}



==> _packages.tex <==

\usepackage{times}
\usepackage{microtype}
\usepackage{epsfig}
\usepackage[table,xcdraw]{xcolor}
\usepackage{caption}
\usepackage{float}
\usepackage{placeins}
\usepackage{color, colortbl}
\usepackage{stfloats}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{xstring}
\usepackage{multirow}
\usepackage{xspace}
\usepackage{url}
\usepackage{subcaption}
\usepackage{svg}
\usepackage[hang,flushmargin]{footmisc}

\ifcamera \usepackage[accsupp]{axessibility} \fi

\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{duckuments}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{float}
\usepackage[10pt]{moresize}

\usepackage{color}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{times}

\usepackage{comment}




\usepackage{pifont}

\usepackage{microtype}
\frenchspacing

\usepackage[font=smaller]{caption}
\usepackage{tabularx}
\usepackage{adjustbox}
\usepackage{array}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{float,wrapfig}
\usepackage{makecell}
\usepackage{hhline}
\usepackage{multirow}
\usepackage{subcaption} %
\usepackage[percent]{overpic}
\usepackage{graphbox}
\usepackage{diagbox}
\usepackage{stmaryrd}


\usepackage{amsmath,amsfonts,amssymb}
\usepackage{bm}
\usepackage{nicefrac}
\usepackage{microtype}
\usepackage{dsfont}
\usepackage{changepage}
\usepackage{extramarks}
\usepackage{fancyhdr}
\usepackage{setspace}
\usepackage{soul}
\usepackage{xspace}
\usepackage{hhline}

\usepackage[colorlinks=true,citecolor=blue,pagebackref=true]{hyperref}



\usepackage{enumitem}
\usepackage[title]{appendix}

\usepackage{arydshln}

\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}


==> cvpr_header.tex <==
\ifreview \usepackage[review]{cvpr} \fi
\ifarxiv \usepackage[pagenumbers]{cvpr} \fi
\ifrebuttal \usepackage[rebuttal]{cvpr} \fi
\ifcamera \usepackage{cvpr} \fi

\makeatletter
\@namedef{ver@everyshi.sty}{}
\makeatother
\usepackage{tikz}

\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}

\input{_packages}
\input{_macros}  %

\usepackage{xr-hyper}

\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}

\makeatother
\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}
\usepackage[capitalize]{cleveref}

\crefname{section}{Sec.}{Secs.}
\crefname{table}{Table}{Tables}
\crefname{figure}{Fig.}{Figs.}

\frenchspacing


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/1ipc_ConvNet_half.tex <==
\begin{table}[]
\vspace{-0.2cm}

\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
Alg.                                              & Distil. Space & ImNet-A            & ImNet-B            & ImNet-C            & ImNet-D            & ImNet-E           \\\midrule
                                                          & Pixel         & 51.7{\color{gray}$\pm$0.2} & 53.3{\color{gray}$\pm$1.0 }& 48.0{\color{gray}$\pm$0.7 }& 43.0{\color{gray}$\pm$0.6} & 39.5{\color{gray}$\pm$0.9 }\\
\multirow{-2}{*}{\mtt{}}                       & \texttt{GLaD} (Ours)    & 50.7{\color{gray}$\pm$0.4}& 51.9{\color{gray}$\pm$1.3 }& 44.9{\color{gray}$\pm$0.4} & 39.9{\color{gray}$\pm$1.7 }& 37.6{\color{gray}$\pm$0.7}\\ \midrule
\cellcolor[HTML]{FFFFFF}                                  & Pixel         & 43.2{\color{gray}$\pm$0.6 }& 47.2{\color{gray}$\pm$0.7} & 41.3{\color{gray}$\pm$0.7 }& 34.3{\color{gray}$\pm$1.5} & 34.9{\color{gray}$\pm$1.5}  \\
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\dc{}} & \texttt{GLaD} (Ours)    & 44.1{\color{gray}$\pm$2.4 }& 49.2{\color{gray}$\pm$1.1} & 42.0{\color{gray}$\pm$0.6} & 35.6{\color{gray}$\pm$0.9} & 35.8{\color{gray}$\pm$0.9} \\ \midrule
\cellcolor[HTML]{FFFFFF}                                  & Pixel         & 39.4{\color{gray}$\pm$1.8 }& 40.9{\color{gray}$\pm$1.7} & 39.0{\color{gray}$\pm$1.3} & 30.8{\color{gray}$\pm$0.9} & 27.0{\color{gray}$\pm$0.8} \\
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\dm{}} & \texttt{GLaD} (Ours)   & 41.0{\color{gray}$\pm$1.5} & 42.9{\color{gray}$\pm$1.9} & 39.4{\color{gray}$\pm$0.7 }& 33.2{\color{gray}$\pm$1.4} & 30.3{\color{gray}$\pm$1.3}
\end{tabular}
}
\caption{
Performance on ConvNet (architecture used to distill).
}
\label{tab:convnet}
\end{table}

==> tables/reg.tex <==
\begin{table}[]
\vspace{-0.2cm}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
Alg.                                    & Distil. Space  & ImNet-A                             & ImNet-B                             & ImNet-C                             & ImNet-D                             & ImNet-E                             \\ \midrule
                                                & Pixel          & 33.4{\color{gray}$\pm$1.5}          & 34.0{\color{gray}$\pm$3.4}          & 31.4{\color{gray}$\pm$3.4}          & 27.7{\color{gray}$\pm$2.7}          & 24.9{\color{gray}$\pm$1.8}          \\
                                                & Pixel+Reg.     & 36.9{\color{gray}$\pm$2.8}          & 35.9{\color{gray}$\pm$1.4}          & 32.5{\color{gray}$\pm$1.5}          & 28.1{\color{gray}$\pm$1.5}          & 24.9{\color{gray}$\pm$1.7}          \\
\multirow{-3}{*}{\mtt{}}                        & \glad{} (Ours) & \textbf{39.9{\color{gray}$\pm$1.2}} & \textbf{39.4{\color{gray}$\pm$1.3}} & \textbf{34.9{\color{gray}$\pm$1.1}} & \textbf{30.4{\color{gray}$\pm$1.5}} & \textbf{29.0{\color{gray}$\pm$1.1}} \\ \midrule
\cellcolor[HTML]{FFFFFF}                        & Pixel          & 38.7{\color{gray}$\pm$4.2}          & 38.7{\color{gray}$\pm$1.0}          & 33.3{\color{gray}$\pm$1.9}          & 26.4{\color{gray}$\pm$1.1}          & 27.4{\color{gray}$\pm$0.9}          \\
\cellcolor[HTML]{FFFFFF}                        & Pixel+Reg.     & 38.9{\color{gray}$\pm$4.8}          & 39.5{\color{gray}$\pm$1.6}          & 32.3{\color{gray}$\pm$1.2}          & 26.2{\color{gray}$\pm$1.3}          & 28.6{\color{gray}$\pm$1.2}          \\
\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}\dc{}} & \glad{} (Ours) & \textbf{41.8{\color{gray}$\pm$1.7}} & \textbf{42.1{\color{gray}$\pm$1.2}} & \textbf{35.8{\color{gray}$\pm$1.4}} & \textbf{28.0{\color{gray}$\pm$0.8}} & \textbf{29.3{\color{gray}$\pm$1.3}}
\end{tabular}
}

\caption{\glad{} compared to total variation and L2 regularization.
}
\label{tab:reg}
\end{table}
